Balancing Minimum Spanning and Shortest Path Trees

This paper give a simple linear-time algorithm that, given a weighted digraph, finds a spanning tree that simultaneously approximates a shortest-path tree and a minimum spanning tree. The algorithm provides a continuous trade-off: given the two trees and epsilon > 0, the algorithm returns a spanning tree in which the distance between any vertex and the root of the shortest-path tree is at most 1+epsilon times the shortest-path distance, and yet the total weight of the tree is at most 1+2/epsilon times the weight of a minimum spanning tree. This is the best tradeoff possible. The paper also describes a fast parallel implementation.

==> NPC-fig.tex <==
\setlength{\unitlength}{0.00083333in}
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
{\renewcommand{\dashlinestretch}{30}
\begin{picture}(5604,4582)(0,-10)
\put(218,4350){\ellipse{420}{420}}
\put(2933,3750){\ellipse{420}{420}}
\put(608,2235){\ellipse{420}{420}}
\put(1493,2220){\ellipse{420}{420}}
\put(2408,2235){\ellipse{420}{420}}
\put(3293,2235){\ellipse{420}{420}}
\put(4208,2235){\ellipse{420}{420}}
\put(5093,2235){\ellipse{420}{420}}
\path(3068,1410)(2693,1320)
\path(2802.685,1377.176)(2693.000,1320.000)(2816.688,1318.833)
\path(3068,1350)(2963,1245)
\path(3026.640,1351.066)(2963.000,1245.000)(3069.066,1308.640)
\path(3248,1350)(3488,1275)
\path(3364.514,1282.159)(3488.000,1275.000)(3382.411,1339.427)
\path(4703,1440)(4583,1320)
\path(4646.640,1426.066)(4583.000,1320.000)(4689.066,1383.640)
\path(4643,1500)(3983,1290)
\path(4088.255,1354.972)(3983.000,1290.000)(4106.447,1297.797)
\path(4808,1500)(4958,1470)
\path(4834.447,1464.117)(4958.000,1470.000)(4846.214,1522.951)
\path(1463,1455)(1838,1290)
\path(1716.080,1310.869)(1838.000,1290.000)(1740.244,1365.788)
\path(1463,1470)(1688,1485)
\path(1570.261,1447.084)(1688.000,1485.000)(1566.270,1506.951)
\path(1283,1470)(1073,1380)
\path(1171.480,1454.845)(1073.000,1380.000)(1195.115,1399.696)
\path(443,3585)(98,3510)
\path(208.888,3564.807)(98.000,3510.000)(221.634,3506.176)
\path(443,3585)(173,3600)
\path(294.479,3623.297)(173.000,3600.000)(291.151,3563.390)
\path(413,3600)(233,3675)
\path(355.308,3656.538)(233.000,3675.000)(332.231,3601.154)
\dashline{60.000}(4418,2220)(4883,2220)
\dashline{60.000}(2618,2220)(3083,2220)
\dashline{60.000}(818,2220)(1283,2220)
\dashline{60.000}(428,4290)(2723,3795)
\path(5063,2025)(4928,1185)
\path(3398,1185)(4928,2115)
\path(4028,2145)(1688,1185)
\path(3458,2100)(4673,1185)
\path(2513,2055)(2963,1185)
\path(2258,2100)(1448,1185)
\path(1628,2070)(2813,1185)
\path(803,2145)(4148,1185)
\path(1148,1185)(683,2040)
\path(3128,3660)(4943,2355)
\path(3098,3600)(4088,2400)
\path(3023,3555)(3248,2445)
\path(2843,3555)(2483,2430)
\path(2768,3615)(1643,2370)
\path(2738,3660)(773,2355)
\path(563,1185)(563,855)(1973,855)
        (1973,1185)(563,1185)
\path(2348,1185)(2348,855)(3758,855)
        (3758,1185)(2348,1185)
\path(4148,1185)(4148,855)(5558,855)
        (5558,1185)(4148,1185)
\path(233,4140)(233,4139)(233,4137)
        (233,4134)(233,4128)(233,4120)
        (233,4109)(233,4095)(233,4077)
        (233,4056)(233,4031)(232,4002)
        (232,3969)(232,3931)(232,3890)
        (232,3845)(232,3797)(232,3744)
        (232,3689)(232,3630)(232,3568)
        (232,3504)(232,3438)(232,3369)
        (232,3299)(232,3227)(232,3153)
        (233,3079)(233,3003)(233,2927)
        (234,2851)(234,2774)(235,2697)
        (236,2619)(236,2542)(237,2464)
        (238,2386)(240,2309)(241,2231)
        (242,2154)(244,2077)(246,2000)
        (248,1923)(250,1846)(252,1769)
        (254,1692)(257,1616)(260,1540)
        (263,1465)(267,1390)(271,1317)
        (275,1244)(279,1174)(283,1105)
        (288,1038)(293,975)(299,903)
        (306,836)(312,776)(319,722)
        (325,675)(331,634)(337,598)
        (342,569)(347,545)(351,526)
        (356,511)(359,501)(363,495)
        (366,493)(368,493)(371,497)
        (373,503)(374,511)(376,521)
        (378,533)(379,546)(380,559)
        (382,574)(383,589)(385,604)
        (386,619)(388,633)(390,648)
        (392,661)(395,674)(398,686)
        (402,697)(406,706)(410,714)
        (416,720)(422,725)(428,728)
        (435,729)(443,729)(452,727)
        (462,723)(472,718)(482,712)
        (494,705)(506,698)(518,690)
        (547,674)(574,660)(599,649)
        (620,640)(638,634)(651,628)
        (662,624)(671,621)(678,619)
        (684,617)(691,616)(698,615)
        (707,614)(718,614)(733,614)
        (751,614)(774,616)(801,619)
        (831,623)(863,630)(898,641)
        (931,654)(961,669)(988,684)
        (1013,701)(1035,718)(1055,736)
        (1075,754)(1092,772)(1108,790)
        (1123,806)(1136,821)(1146,833)
        (1154,843)(1159,849)(1162,853)(1163,855)
\path(188,4140)(188,4139)(188,4137)
        (188,4134)(188,4129)(187,4121)
        (187,4110)(186,4096)(185,4079)
        (185,4058)(184,4033)(183,4005)
        (181,3972)(180,3936)(178,3896)
        (177,3852)(175,3804)(173,3753)
        (171,3698)(169,3640)(167,3580)
        (165,3517)(163,3451)(161,3384)
        (160,3314)(158,3243)(156,3171)
        (154,3097)(153,3022)(151,2947)
        (150,2871)(149,2794)(148,2717)
        (147,2640)(147,2562)(147,2485)
        (147,2407)(147,2329)(148,2250)
        (149,2172)(150,2093)(152,2015)
        (154,1936)(157,1857)(160,1777)
        (164,1698)(168,1619)(173,1539)
        (178,1460)(184,1381)(190,1303)
        (197,1225)(205,1148)(214,1073)
        (223,1000)(233,930)(249,832)
        (265,743)(281,662)(297,590)
        (313,528)(328,475)(341,430)
        (353,393)(364,364)(374,342)
        (383,326)(390,315)(397,310)
        (403,308)(407,310)(412,314)
        (416,321)(419,330)(423,340)
        (427,351)(431,361)(436,372)
        (442,381)(448,390)(456,397)
        (466,402)(477,406)(490,406)
        (506,405)(523,400)(544,393)
        (567,383)(592,370)(621,356)
        (652,339)(685,321)(721,303)
        (758,285)(806,265)(855,248)
        (901,233)(943,221)(982,211)
        (1017,203)(1046,197)(1072,192)
        (1093,189)(1111,186)(1125,185)
        (1137,184)(1147,183)(1156,183)
        (1164,184)(1173,185)(1182,186)
        (1193,188)(1207,190)(1224,193)
        (1244,196)(1269,200)(1300,205)
        (1336,211)(1378,219)(1426,228)
        (1481,239)(1541,252)(1605,267)
        (1673,285)(1734,303)(1794,322)
        (1853,342)(1911,363)(1966,385)
        (2020,407)(2072,429)(2121,452)
        (2169,474)(2216,497)(2261,520)
        (2305,543)(2347,567)(2389,590)
        (2429,613)(2469,636)(2507,659)
        (2544,681)(2579,703)(2613,724)
        (2644,744)(2674,763)(2701,781)
        (2725,796)(2746,810)(2764,822)
        (2779,832)(2791,840)(2800,846)
        (2806,850)(2810,853)(2812,854)(2813,855)
\path(143,4155)(143,4154)(143,4152)
        (142,4149)(142,4143)(141,4136)
        (140,4125)(139,4111)(138,4094)
        (136,4073)(134,4048)(132,4020)
        (129,3987)(126,3951)(123,3911)
        (120,3868)(116,3821)(112,3770)
        (108,3717)(104,3660)(100,3601)
        (96,3539)(91,3475)(87,3409)
        (83,3342)(78,3273)(74,3202)
        (70,3131)(66,3059)(62,2986)
        (59,2912)(55,2838)(52,2763)
        (49,2688)(47,2612)(45,2536)
        (43,2460)(41,2383)(40,2306)
        (40,2228)(39,2150)(40,2071)
        (41,1992)(42,1912)(45,1831)
        (47,1751)(51,1669)(55,1588)
        (60,1507)(66,1425)(73,1344)
        (80,1265)(89,1186)(98,1110)
        (111,1016)(125,928)(139,846)
        (152,770)(164,702)(175,641)
        (184,587)(191,539)(197,498)
        (201,463)(203,434)(203,409)
        (202,390)(199,374)(195,362)
        (190,354)(184,348)(177,344)
        (170,342)(163,341)(155,341)
        (149,342)(143,343)(138,344)
        (135,344)(133,343)(134,341)
        (137,338)(144,333)(153,326)
        (167,318)(185,307)(207,293)
        (235,278)(268,260)(306,241)
        (351,219)(403,197)(460,173)
        (524,150)(593,126)(668,105)
        (735,89)(803,74)(873,62)
        (944,51)(1014,42)(1082,34)
        (1149,27)(1214,22)(1276,18)
        (1336,15)(1393,13)(1447,12)
        (1498,12)(1546,13)(1592,14)
        (1635,15)(1676,17)(1715,20)
        (1752,23)(1787,26)(1821,30)
        (1854,33)(1886,37)(1918,42)
        (1949,46)(1981,51)(2013,56)
        (2045,61)(2079,66)(2113,71)
        (2150,77)(2188,83)(2228,89)
        (2271,95)(2317,102)(2365,109)
        (2417,116)(2472,123)(2530,131)
        (2591,139)(2656,148)(2725,158)
        (2796,167)(2871,178)(2948,189)
        (3028,201)(3109,213)(3191,226)
        (3272,240)(3353,255)(3461,276)
        (3564,299)(3661,322)(3750,345)
        (3833,368)(3910,392)(3979,415)
        (4044,438)(4102,461)(4156,484)
        (4206,507)(4252,530)(4294,552)
        (4333,575)(4368,597)(4402,619)
        (4433,641)(4461,663)(4487,684)
        (4512,704)(4534,724)(4554,743)
        (4573,761)(4589,777)(4603,792)
        (4616,806)(4627,818)(4635,828)
        (4643,836)(4648,843)(4652,848)
        (4655,851)(4657,853)(4658,854)(4658,855)
\put(4148,2715){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\A}}}}}
\put(3008,2730){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\A}}}}}
\put(1088,2730){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\A}}}}}
\put(3563,2715){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\A}}}}}
\put(1763,2730){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\A}}}}}
\put(4673,1470){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\B}}}}}
\put(473,3570){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\W}}}}}
\put(4583,2250){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\E}}}}}
\put(2783,2250){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\E}}}}}
\put(3113,1365){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\B}}}}}
\put(1358,1440){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\B}}}}}
\put(2393,2730){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\A}}}}}
\put(983,2265){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\E}}}}}
\put(1493,4110){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\D}}}}}
\put(2273,2160){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\literalC }}}}}
\put(143,4305){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\rootA }}}}}
\put(2858,3705){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\rootB }}}}}
\put(473,2160){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\literalA }}}}}
\put(1358,2160){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\literalB }}}}}
\put(3158,2160){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\literalD }}}}}
\put(4073,2160){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\literalE }}}}}
\put(4958,2160){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\literalF }}}}}
\put(803,960){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\clauseA }}}}}
\put(2558,960){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\clauseB }}}}}
\put(4358,960){\makebox(0,0)[lb]{\smash{{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}\clauseC }}}}}
\end{picture}
}


==> ex2.tex <==
\begin{picture}(0,0)%
\includegraphics{ex2.eps}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(6649,6700)(121,-6206)
\end{picture}


==> leadEx.tex <==
\begin{picture}(0,0)%
\includegraphics{leadEx.eps}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(6936,5673)(3151,-6941)
\end{picture}


==> parFig.tex <==
\begin{picture}(0,0)%
\includegraphics{parFig.eps}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4126,3670)(1066,-3821)
\end{picture}


==> tight-ex.tex <==
\begin{picture}(0,0)%
\includegraphics{tight-ex.eps}%
\end{picture}%
\setlength{\unitlength}{59204sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(246,139)(197,637)
\put(323,696){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}A}}}
\put(317,667){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}c}}}
\put(319,770){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}r}}}
\put(253,707){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}C}}}
\put(302,649){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}B}}}
\end{picture}

